Hyperparameter Sensitivity in Deep Outlier Detection: Analysis and a Scalable Hyper-Ensemble Solution

Outlier detection (OD) literature exhibits numerous algorithms as it applies to diverse domains. However, given a new detection task, it is unclear how to choose an algorithm to use, nor how to set its hyperparameter(s) (HPs) in unsupervised settings. HP tuning is an ever-growing problem with the arrival of many new detectors based on deep learning, which usually come with a long list of HPs. Surprisingly, the issue of model selection in the outlier mining literature has been "the elephant in the room"; a significant factor in unlocking the utmost potential of deep methods, yet little said or done to systematically tackle the issue. In the first part of this paper, we conduct the first large-scale analysis on the HP sensitivity of deep OD methods, and through more than 35,000 trained models, quantitatively demonstrate that model selection is inevitable. Next, we design a HP-robust and scalable deep hyper-ensemble model called ROBOD that assembles models with varying HP configurations, bypassing the choice paralysis. Importantly, we introduce novel strategies to speed up ensemble training, such as parameter sharing, batch/simultaneous training, and data subsampling, that allow us to train fewer models with fewer parameters. Extensive experiments on both image and tabular datasets show that ROBOD achieves and retains robust, state-of-the-art detection performance as compared to its modern counterparts, while taking only $2$-$10$\% of the time by the naive hyper-ensemble with independent training.

==> 035design_copy.tex <==
\newcommand{\identity}{\mathbbm{1}}
\newcommand{\realR}{\mathbb{R}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bw}{\mathbf{W}}
\newcommand{\bss}{\mathbf{s}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bSS}{\mathbf{S}}

\subsection{Design Strategies for Speeding up Ensemble Training}

\subsubsection{Hyper-ensembling depth: One model for multiple depths}
\label{sssec:dep}
Skipping connections, or shortcut connections, are applied in neural network architectures for various purposes. The most well-known types include ResNet for solving the degradation problem, Stochastic Depth Neural Network as an implicit ensemble of networks of different depths, UNet for biomedical image segmentation, etc. \la{citations. also: Lingxiao, some for oversmoothing? what is the name? }

Due to the ``hourglass'' structure of the AE, skipping one layer in an AE would cause dimensionality mismatch for the next layer. Instead, we create long shortcuts by skipping the middle layers while keeping the outer encoder-decoder pairs symmetrically, and refer to this architecture as \aes.  

 An illustration of hyper-ensembling depth can be found in Figure \ref{fig:chart}; see e.g. the \aes denoted by $f_j$. Given a $2L$-layer \aes ($L$ encoder and $L$ decoder layers), there are $2L$ trainable weight matrices. For input $\mathcal{D}$, we generate $L$ outputs by allowing the input to pass through the outermost encoder-decoder pair (which we denote as $AE\text{-}2$), the two outermost encoder-decoder pairs ($AE\text{-}4$), and so on, until the full structure ($AE\text{-}2L$) is traversed by the input.
 In effect, this trains $L$ different AEs under one \aes model.
  Then, the overall loss $\mathcal{L}_{\text{\aes}}$ of the depth-hyper-ensembling \aes is the summation of %$L-1$ autoencoder members' 
  the member AEs'
  reconstruction errors (denoted $\Delta Err$). Eq. \eqref{eq:AEs_loss} gives an example of the loss function for a $6$-layer \aes as shown in Figure \ref{fig:chart},
\begin{equation}
 \scalemath{0.975}{
	\label{eq:AEs_loss}	
	\mathcal{L}_{\text{\aes}}
	=  \Delta Err_{AE\text{-}2}(\mathcal{D}; [\mathbf{W}_1\text{:}\mathbf{W}_2]) 
	+
	 \Delta Err_{AE\text{-}4}(\mathcal{D}; [\mathbf{W}_1\text{:}\mathbf{W}_4]) 
	 +
	 \Delta Err_{AE\text{-}6}(\mathcal{D}; [\mathbf{W}_1\text{:}\mathbf{W}_6]) 
%	+	RecErr_{AE\text{-}8}(\mathcal{D}; [\mathbf{W}_1\text{:}\mathbf{W}_8]) 
}
\end{equation}
\la{do we need to clarify notation $[\mathbf{W}_y\text{:}\mathbf{W}_{y'}]$ above?}
Similar to ResNet with stochastic depth \la{maybe drop}, \aes is an implicit hyper-ensemble which allows simultaneous/joint training of AEs with various depths. It is computationally efficient thanks to parameter sharing, as the outer layers' weights are reused and tuned among different members. Each ensemble member can also play a regularization effect on the anomaly score (the reconstruction error), to prevent an AE from producing low scores for anomalies due to overfitting. (See Appx. \textcolor{red}{Sec. \ref{}}). 

\subsubsection{ Hyper-ensembling width: Zero-masked joint training}
\label{sssec:wid}
BatchEnsemble \cite{conf/iclr/WenTB20} (BE) is a state-of-the-art parameter-efficient deep ensemble training approach. However, 
off-the-shelf, it does not allow for {\em hyper-}ensebling, that is, all models in the batch are trained with the same HP configuration, and share equal size parameters.
 Our approach builds on BE, adapting it to simultaneously train varying-width \aes with shared parameters.

First, we briefly review the BE architecture with $K$ AEs. For a specific layer in BE, weight $\bw \in \realR^{m\times r}$ is shared across all $K$ individual members, while each member $i$ maintains two trainable rank-1 vectors: $\br_i \in \realR^m$ and $\bss_i \in \realR^r$. The outer product ($\cdot$) of $ \br_i$ and  $\bss_i^T$ creates a ``mask'' (a matrix in $\realR^{m\times r}$) onto the shared weight $\bw$ and generates individual weight $\overline{\bw_i}$. For the input mini-batch  $\mathbf{X}_i \in \realR^{m \times n}$, the forward propagation computation is \la{need it to be $\bss_i \cdot \br_i^T$ as in Fig.3}
\begin{equation}
	\Phi \big(\overline{\bw_i}^T \; \mathbf{X}_i \big) = \Phi \big( (\bw \circ ( \br_i \cdot \bss_i^T ))^T \; \mathbf{X}_i \big) = \Phi \big( (\mathbf{X}_i \circ \br_i) \bw \circ \bss_i \big) \;,
	\label{eq:be}
\end{equation}
where $\Phi$ is the activation function, $\circ$ is the element-wise product, and $\br_i$ and $\bss_i$ are broadcasted row-wise or column-wise depending on the shapes at play. To vectorize the calculation for all $K$ members in the ensemble, two matrices $\bR \in \realR^{K \times m}$ and $\bSS \in \realR^{K \times r}$ are constructed with rows of $\br_i$ and $\bss_i$, respectively. Thus, for the input %$\mathbf{X} \in \realR ^{Kr \times m}$, 
$\mathbf{X} \in \realR ^{Km \times n}$, the BE layer computes the next layer as
\begin{equation}
	\Phi \big( (\mathbf{X} \circ {\bR}) \bw \circ \bSS \big) \;.
\end{equation}
Since $\mathbf{X}$ is composed of $K$ mini-batching $\mathbf{X}_i$'s tiling up, each member can utilize a different mini-batch of input. The $K$ members are training simultaneously in parallel using one forward pass, thus relieving the memory and computational burden of traditional ensemble methods.

While BE itself is not a hyper-ensemble, we can leverage this architecture to aggregate networks of different widths, also in an efficient way. The widths of a neural network layer correspond to the rows in the weight matrix. For a specific layer, instead of directly operating on $\bw$, we instead initialize a zero-one masking vector $\mathbf{\balpha}_i \in \{0,1\}^r$. $\mathbf{\balpha}_i$ is to element-wise multiply with the $\bss_i \in \realR^r$, such that the operation $\bw \circ \br_i \cdot (\bss_i^T \circ \mathbf{\balpha}_i^T)$ will create a masking matrix of size $(m \times r)$ and sparsify the individual weight $\overline{\bw_i}$ by allowing zero'ed-out rows. In vectorized notation, the matrix $\mathbf{A} \in \{0,1 \}^{K \times r}$ is composed of $K$ distinct masking vectors. Then, the zero-masked BE forward propagation becomes
\begin{equation}
	\Phi \big( \mathbf{X} \circ \bR ) \bw \circ (\bSS \circ \mathbf{A}) \big)\;.
\end{equation}
Sparsifying neural networks has been shown to decrease storage and improve training efficiency, % performances of the neural network, 
with many algorithms built to wisely prune the neural network \textcolor{red}{citation}. While zero-masked BE is similar to creating neural networks of varying density, our main goal is to obtain models with different widths (i.e. hidden sizes), such that when trained under BE, creates a width-hyper-ensemble.
%reduce the search effort among various neural network widths. 
Specifically, we construct the zero-masked BE layer with the maximum width and specify the zeros in respective $\mathbf{\balpha}$ vectors,  such that the masked-out individual weights correspond to varying-width models. 

The zero-masked BE is also computationally efficient, as $\mathbf{A}$ is fixed throughout training. The element-wise product of the masking incurs little extra time during forward and backward propagation, while all the (rank-1) vectors are cheap to store compared to storing individual weight matrices as in traditional ensemble training.

\subsubsection{Further speed up by subsampling}
As shown in Eq. \ref{eq:be}, BE allows mini-batching, where each data point can be used by one or several different ensemble members. This makes BE a natural fit to subsampling, which further expedites the training procedure. Specifically, 
we create $\{\mathbf{X}_i^{in}, \mathbf{X}_i^{out} \}_{i=1}^K$ splits of the overall training data, where
for each member $i$, we divide the training data into $\mathbf{X}_i^{in}$ and $\mathbf{X}_i^{out} = \mathbf{X}_i / \mathbf{X}_i^{in}$ and solely train on mini-batches from $\mathbf{X}_i^{in}$. 

\subsubsection{\method: the overall hyper-ensemble}
%In this section, we introduce ROBOD architecture and how to ensemble among different hyper-parameter settings with anomaly scoring function. Let $\mathbf{\lambda}_i$ denote a vector of one hyper-parameter configuration for an auto-encoder with function $f$, and trainable parameters $\mathbf{\theta}_i$. For each individual autoencoder, it takes input $\mathbf{x} \in \realR^m $ into a reduced space and tries to reconstruct $\mathbf{x}$, using the data reconstruction error as the anomaly score function. 

Let us denote by
$H$ the total number of hyperparameters (HPs) for the \aes, where
we define a grid of values for each HP. For the two HPs, \dep and \wid, we specify the \aes with the largest depth value (following Sec. \ref{sssec:dep}, say $2L$) in the grid and leverage the skip connections to obtain the smaller-depth AEs.
Similarly, we specify each \aes in the zero-masked BE with the largest width value (following Sec. \ref{sssec:wid}, say $K$) in the grid and leverage the zero-masking to obtain other, smaller-width AEs.



\la{what is $K$ equal to exactly? All configurations? In 4.2.2 it is the number of \aes models in the (zero-masked) BE, but there are more than $K$ models in total since each \aes itself is an ensemble (of depths). So for $2L$-layer \aes, it should be $K*L$ models overall, right?}

%Assuming $\mathbf{\lambda}_i$ belongs to a subset $S$, where elements in $S$ are potential hyper-parameter configurations, and $|S| = K$. Thus, we need to train $K$ individual autoencoders with the aggregated anomaly scoring function for $i \in \{1,...K \}$:
%
%\begin{equation}
%	s(\mathbf{x}) = \frac{1}{K}\sum_{i=1}^{K}{s_i(\mathbf{x})} \text{    ,where  } s_i(\mathbf{x}) = \lVert  \mathbf{x} - f_{\mathbf{\theta}_i}(\mathbf{x}; {\mathbf{\lambda}_i})  \rVert^2
%\end{equation}





Since we have $\{\mathbf{X}_i^{in}, \mathbf{X}_i^{out} \}_{i=1}^K$ splits of the training data, we can compute the out-of-sample\footnote{In the inductive OD setting (see Sec. \ref{sec:related}), a point is scored by all ensemble members.}
\la{foonote needed right?} anomaly score for a point $\mathbf{x}$ as
\begin{equation}
\scalemath{0.9}{
	s(\mathbf{x}) = \frac{1}{K'} \sum_{i=1}^{K} \identity (\mathbf{x} \in \mathbf{X}_i^{out}) s_i(\mathbf{x})\;, \;\; \text{where} \; s_i(\mathbf{x}) = \sum_{d=1}^L \lVert  \mathbf{x} - f_i^{(AE-2d)}(\mathbf{x}; {\bm{\lambda}_{i,d}})  \rVert^2, \; K' = L  \sum_{i=1}^{K} \identity (\mathbf{x} \in \mathbf{X}_i^{out})
}
\end{equation}
%\begin{equation}
%\scalemath{0.925}{
%	s(\mathbf{x}) = \frac{1}{K'} \sum_{i=1}^{K} \identity (\mathbf{x} \in \mathbf{X}_i^{out}) s_i(\mathbf{x})\;, \;\; \text{where} \; s_i(\mathbf{x}) = \sum_{d=1}^L \lVert  \mathbf{x} - f_{\bm{\theta}_i}(\mathbf{x}; {\bm{\lambda}_i})  \rVert^2, \; K' =  \sum_{i=1}^{K} \identity (\mathbf{x} \in \mathbf{X}_i^{out})
%}
%\end{equation}
\la{score should be avg'ed over varying-depth AEs, too. Should be $K*L$ models overall.}
where $f_i$ is the $i$'th \aes member, $\bm{\lambda}_i$ is a vector depicting a specific configuration of all HPs for \aes member $i$, and $\bm{\theta}_i$ denotes all its trainable parameters. \la{should we add a sentence like: This offers the advantage of scoring an out-of-sample outlier accurately in cases when the model has overfit to the in-sample outliers, assuming the in-sample outliers are different type.}


\la{average s(x) values across all B trained zero-masked BEs.}


For example, hyper-parameter configurations can be: \textit{number of layer} = $[2,3,4]$, \textit{learning rate} = $[1e^{-3}, 5e^{-4}]$, \textit{dropout rate} = $[0.0, 0.2]$. $\mathbf{\lambda}_i$ can be a specific hyper-parameter configuration with \textit{number of layer} $= 2$, \textit{learning rate}  $= 1e^{-3}$, \textit{dropout rate}  $= 0.0$. Since $|S| = 12$, a hyper-ensemble averages scores from $12$ different $f_{\mathbf{\theta}_i}(\boldsymbol{\cdot} ;\mathbf{\lambda}_i)$.



==> 05experiments.tex <==
%!TEX root = paper.tex


We conduct experiments to answer the following: \textbf{Q1.} How does \method compare to state-of-the-art OD methods? \textbf{Q2.} How much does \method's performance vary by initialization? 
\textbf{Q3.} What are the savings in running time and memory usage compared to the independent/na\"ive hyper-ensemble?


{\bf Baselines.~} 


{\bf Datasets.~} 

\input{TABLE/datasets.tex}


{\bf Configurations.~}



\input{TABLE/comparison.tex}



%\input{TABLE/recommended.tex}
 


We evaluate the Vanilla-ROBOD and ROBOD with several deep methods, on two image datasets, MNIST and CIFAR10, and three tabular datasets. The brief overview of dataset preparation and dataset statistics can be found \textcolor{red}{list appendix or section number}. For evaluation, we use the Area under the ROC Curve (AUC) score, as well as comparing the time and memory-storage across the methods, on a server with three A6000 GPUs.

\subsection{Setup}
\label{expsec:setup}

%\vspace{-0.1in}
\subsubsection{\bf Baselines.~} 
The shallow method we include in comparison is Isolation Forest \textcolor{red}{citation}. We choose Isolation Forest because it is an ensemble based method in anomaly detection, isolating the outliers among the decision trees. We set a grid search of $\textit{num of trees} \in [50,100,200,500]$ and the subsampling $\textit{max samples} \in [64,128,256,512]$.

The deep methods we are comparing to are (i)VanillaAE, (ii) RDA, (iii) DeepSVDD, (iv) RandNet. \textcolor{red}{citation} These three methods are recent deep anomaly detectors which are either distance-based or using autoencoder as the backbone structure. Since they are deep-learning based methods, the classification accuracies are varied to different hyper-parameter choices. In addition, RandNet is also en ensemble method with sparse neural networks and random initialization. 

In Appendix \textcolor{red}{which?}, we recognize the common network architecture and optimization hyper-parameters among these baseline methods. In addition, there are algorithm choices and algorithm-specific hyper-parameters for different deep methods: (i) RDA applies $\lambda$  as a $l1$-penalization term on the sparsity of outlier, inner iteration, and outer iteration for alternative updating autoencoders and outlier matrix. (ii) DeepSVDD pre-trains weights on autoencoder before initialize centroid $c$, so we can further grid search on pre-training iteration and its learning rate. An additional hyper-parameter is the slope of the leaky-Relu activation. (iv) For RandNet, we can also perform search on number of network models,  adaptive sampling ratio, and layer-wise pretraining epochs.



\subsubsection{\bf ROBOD.~}%{\bf}
In hyper-ensemble (VanillaROBOD), we refer to the predictions we have acquired from VanillaAE and give anomaly scores to data points as the average over whole predictions. ROBOD conducts a structure ensemble over the neural network lengths and widths. For fair comparison with VanillaAE results, we set the maximum number of layers as $6$, similar to VanillaAE's maximum NN depth. IN each BatchEnsemble AE-s unit, we allow number of models to $8$, which corresponds to different hidden unit widths we have in grid-searching VanillaAE's network widths. We denote $ROBOD$ \textcolor{red}{a new command for the method} as the model without subsampling, and $ROBOD_{sub-s}$ denotes the model with $s$ subsample rate. Refer to Appendix \textcolor{red}{appendix number?} for details.


\subsection{Results}
\label{expsec:results}
.


%\begin{figure}[!ht]
%	\centering
%	\begin{tabular}{cccc}
%		\hspace{-0.25in}
%		\includegraphics[width=0.275\textwidth]{plots/auc_time_mnist8_no_legend.png} &
%		\hspace{-0.2in}
%		\includegraphics[width=0.275\textwidth]{plots/auc_time_lympho_no_legend.png} &
%		\hspace{-0.1in}
%		\includegraphics[width=0.275\textwidth]{plots/auc_time_mnist8_no_legend.png} &
%		\hspace{-0.2in}
%		\includegraphics[width=0.275\textwidth]{plots/auc_time_lympho_no_legend.png} \\
%		%
%	\end{tabular}
%	\caption{\label{fig:scatter} Runtime vs AUC }
%\end{figure}
%
%- running time by num of models $m$
%
%
%\begin{figure}[!ht]
%	\vspace{-0.1in}
%	\centering
%	%\includegraphics[width=0.99\linewidth]{FIG/selection}
%	\vspace{-0.1in}
%	\caption{caption \label{fig:selection}}
%		\vspace{-0.15in}
%\end{figure}
%



==> TABLE/recommended.tex <==
\begin{table}[ht!]
    \centering
    \caption{Percentage AUC score of baseline methods, with each utilizes the recommended setting mentioned in the literature. Since the backbone of DeepSVDD is convolutional autoencoders, it does not report results on tabular data.  }
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrr|rr|rrr}
		\toprule &  MNIST- & MNIST- & MNIST- & CIFAR10- & CIFAR10- & Cardio & Thyroid & Lympho \\
		& Digit 4 & Digit 5 & Digit 8 & Airplanes & Automobiles & & & \\
		\midrule
		IF & \\
        RDA &84.2$\pm$2.7& 74.7$\pm$8.6& 87.3$\pm$2.4& 65.7$\pm$5.5 & 60.0$\pm$2.4 & 70.5$\pm$9.3 & 81.5$\pm$4.7 & 71.2$\pm$11.8\\
        DeepSVDD & 84.0$\pm$2.1 & 76.2 $\pm$1.5 & 86.2$\pm$1.6 & 57.8$\pm$2.6 & 62.3$\pm$1.7 & -& - & -\\
        RandNet &84.9$\pm$3.1 &78.9$\pm$2.5 & 86.1$\pm$1.7 & && 87.8$\pm$4.5 & 83.7$\pm$3.6 & 91.8$\pm$7.8 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:recommend_AUC}
\end{table}
